Octavius: Mitigating Task Interference in MLLMs via LoRA-MoE

Recent studies have demonstrated Large Language Models (LLMs) can extend their zero-shot generalization capabilities to multimodal learning through instruction tuning. As more modalities and downstream tasks are introduced, negative conflicts and interference may have a worse impact on performance. While this phenomenon has been overlooked in previous work, we propose a novel and extensible framework, called Octavius, for comprehensive studies and experimentation on multimodal learning with Multimodal Large Language Models (MLLMs). Specifically, we combine the well-known Mixture-of-Experts (MoE) and one of the representative PEFT techniques, i.e., LoRA, designing a novel LLM-based decoder, called LoRA-MoE, for multimodal learning. To the best of our knowledge, we are one of the pioneering efforts to introduce MoE into MLLMs to address this problem. The experimental results (about 20% improvement) have shown the effectiveness and versatility of our design in various 2D and 3D downstream tasks. Code and datasets are available at https://openlamm.github.io/tutorial/.

==> sections/archive/ch1_intro_v2.tex <==
\section{Introduction}
\label{sec:intro}

Multimodal Large Language Models (MLLMs)~\citep{alayrac2022flamingo, huang2023kosmos1, liu2023llava, li2023otter, zhu2023minigpt} have been considered as promising general-purpose interfaces that aim at performing universal multimodal tasks under few-/zero-shot settings.
%
To achieve this goal, apart from leveraging the powerful Large Language Models (LLMs) as the language decoder to generate unified textual responses to different tasks, MLLMs should also learn to perceive general modalities and efficiently fine-tune the MLLMs to align more downstream tasks.
%
Usually, it requires an instruction-following fine-tuning paradigm~\citep{ouyang2022instruction}, which converts multimodal task into a group of instruction-following dialogues, and then fine-tune the LLMs with these dialogues.

Instead of implementing a full fine-tuning scheme, which retains all model parameters, recent MLLMs~\citep{zhang2023llamaadapter, yin2023lamm, ye2023mplug} have attempted to employ the Parameter-Efficient Fine-Tuning (PEFT), \emph{e.g.}, LoRA~\citep{hu2021lora} or Adapters~\citep{houlsby2019adapter}, to efficiently update their models, enabling the MLLMs to acquire out-of-domain knowledge in specific downstream multimodal tasks while preserving their language proficiency.
%
PEFT reduces the reliance on extensive instruction-following datasets, which is particularly useful for fine-tuning with tasks from modalities that have very limited well-annotated data, such as 3D point cloud.
%
Remarkably, these models achieve comparable performance at a low cost in comparison to recent LLaVA~\citep{liu2023llava}, KOSMOS series~\citep{huang2023kosmos1,peng2023kosmos2} and Shikra~\citep{chen2023shikra}, which are learned by full model fine-tuning with a large amount of multimodal instruction-following data.

However, PEFT has to address the crucial tug-of-war problem~\citep{hadsell2020embracing}, where simultaneously learning different tasks may cancel each task-specific optimization out, and ultimately compromise the performance of each downstream task.
%
This problem is much more severe in learning MLLMs.
%
First, the features from the new modalities are not easy to be aligned with each other, as well as compatible with the LLM-based language decoder. 
%
Second, simultaneously learning knowledge at distinct visual granularity in one MLLM model, such as the instance-level perception (\emph{e.g.}, object detection) and logical reasoning (\emph{e.g.}, VQA), may lead to significant interference between each other. 
%
Third, using an LLM-based decoder to predict specific outputs of the multimodal tasks is more complicated than those of the NLP tasks. 


\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/sec1_intro_teaser.pdf}
    \caption{
        \textbf{\mname} is a unified, multimodal large language model with a novel capability to comprehend various tasks across different modalities, including but not limited to 2D captioning, 2D detection, 3D VQA, and 3D dense captioning.
    } 
    \label{fig:intro_teaser}
\end{figure}

\textcolor{red}{
To resolve this issue, we propose \textbf{\dec}, which combines the well-known Mixture-of-Experts (MoE)~\citep{jacobs1991adaptive, jordan1994hierarchical} and one of the representative PEFT techniques, \emph{i.e.}, LoRA~\citep{hu2021lora}.
%
% To resolve this issue, we propose \textbf{\dec} with a sample-based gating strategy, which combines the well-known Mixture-of-Experts (MoE)~\citep{jacobs1991adaptive, jordan1994hierarchical} and one of the representative PEFT techniques, \emph{i.e.}, LoRA~\citep{hu2021lora}.
%
Based on \dec, an LLM-based decoder can efficiently be involved in more downstream tasks and more modalities by learning more LoRA modules.
%
Different from conventional MoE in foundation models~\citep{shazeer2017sparsemoe, lepikhin2020gshard, fedus2022switch, du2022glam}, we adopt a simple yet effective instance-based gate routing scheme, sparsely activating independent LoRA experts with instance-level instructions and further acquiring task-specific knowledge for better aligning different tasks.
}
% Different from conventional MoE in foundation models~\citep{shazeer2017sparsemoe, lepikhin2020gshard, fedus2022switch, du2022glam}, we adopt a simple but effective sample-based gate routing scheme, allowing sparsely-activated LoRA modules to learn task-specific knowledge as an independent expert.
%
Notably, to our best knowledge, we are the first work to introduce MoE into MLLMs to address the tug-of-war problem.

To validate the effectiveness of \dec, in this work, we investigate a more complicated scenario, where the MLLMs should simultaneously learn downstreaming tasks from more additional modalities, such as 2D images and 3D point clouds. 
%
This scenario is especially useful for embodied agents~\citep{duan2022embodiedaisurvey, mu2023embodiedgpt, driess2023palm}.
%
Specifically, in addition to the off-the-shelf image encoder, we design a point cloud encoder called \textbf{\enc}, which provides language-aligned scene-level point cloud representations. 
%
This encoder at first gathers language-aligned point cloud features of each instance~\citep{xue2023ulip} in a scene, which are then aggregated into a scene-level feature based on the attention operation guided by the input instructions.

Based on the aforementioned contributions, we introduce a novel and extensive framework called \textbf{{\mname}},
%
which learns the MLLMs upon the instruction-following datasets adapted from LAMM~\citep{yin2023lamm} and ScanNet~\citep{dai2017scannet}. As shown in Figure~\ref{fig:intro_teaser}, {\mname} can successfully address various 2D/3D vision and language tasks, including but not limited to 2D detection, 2D captioning, 3D VQA, and 3D dense captioning.
%
We conduct various experiments to validate the effectiveness and versatility of our design, improving multiple downstream tasks by about 20\% while increasing only a few trainable parameters.


==> sections/archive/ch2_related_works.tex <==
\section{Related Works}
\label{sec:related_works}

\textbf{Large Language Models (LLMs) \& PEFT.}
%
Recently, Large Language Models (LLMs)~\citep{brown2020language, chowdhery2022palm, chiang2023vicuna, touvron2023llama2} have gained significant attention due to their impressive capabilities in language generation~\citep{zhang2022opt}, in-context learning~\citep{wei2022chain}, and reasoning~\citep{touvron2023llama}.
%
For both data- and compute-efficient adaptation on certain downstream tasks, several PEFT (Parameter-Efficient Fine-Tuning)~\citep{li2021prefix,houlsby2019adapter,karimi2021compacter,hu2021lora} are proposed.
%
For instance, ~\citet{hu2021lora} represents weight updates using two smaller matrices through low-rank decomposition, where original weights are kept frozen while the new update matrices are trained.
%
In this work, we adopt LoRA for efficient MLLMs fine-tuning.

\textbf{Multimodal Large Language Models (MLLMs).}
%
Several recent studies have attempted to extend the capability of LLMs to multimodal tasks.
%
\citet{alayrac2022flamingo, li2023blip2, liu2023llava, zhang2023llamaadapter, yin2023lamm, chen2023shikra, peng2023kosmos2} introduce image modality in LLMs for comprehending 2D visual content. 
%
% \citet{chen2023shikra, peng2023kosmos2} enhance 2D visual understanding through incorporating object localization in images.
%
\citet{hong20233dllm} combines LLMs with 3D modality by rendering point clouds into 2D images and utilizing them to represent 3D visual features. 
%
\citet{driess2023palm, mu2023embodiedgpt, brohan2023rt} establish connections between visual inputs and embodied controls for robotic tasks.
%
% \citet{huang2023kosmos1, su2023pandagpt} consider the integration of audio into LLMs. 
%
Despite its wide range of multimodal applications, the performance degradation caused by interference between tasks and modalities during fine-tuning in MLLMs receives inadequate attention.

\textbf{Mixture-of-Experts (MoE).}
%
Deep MoE models are proposed to increase the number of model parameters without adding computational overhead in the field of computer vision~\citep{riquelme2021scaling, mustafa2022multimodal, shen2023scaling} and natural language processing~\citep{shazeer2017sparsemoe, lepikhin2020gshard, fedus2022switch}. 
%
% A common and critical issue with MoE models is imbalance among experts~\citep{eigen2013imbalance}, which leads the gating network to favor only a few experts and thus under-utilize all experts.
%
% Some researchers~\citep{shazeer2017sparsemoe, zhou2022mixture, wu2022residual} introduce load balancing methods to mitigate this issue.
%
Different from these approaches, we aim to address conflicts between tasks with MoE.
%
Adamix~\citep{wang2022adamix}, an approach related to but distinct from ours, randomly selects experts during training and uses the average weights of these experts in inference, which may be analogous to dropout~\citep{srivastava2014dropout} in certain cases.
%
In this paper, we desire for a dynamic gate routing strategy to automatically calculate the weights of each LoRA expert according to the input instructions, adapting MLLMs for broader multimodal applications.

